Adapting Software Architectures to Machine Learning Challenges

Unique developmental and operational characteristics of ML components as well as their inherent uncertainty demand robust engineering principles are used to ensure their quality. We aim to determine how software systems can be (re-) architected to enable robust integration of ML components. Towards this goal, we conducted a mixed-methods empirical study consisting of (i) a systematic literature review to identify the challenges and their solutions in software architecture for ML, (ii) semi-structured interviews with practitioners to qualitatively complement the initial findings and (iii) a survey to quantitatively validate the challenges and their solutions. We compiled and validated twenty challenges and solutions for (re-) architecting systems with ML components. Our results indicate, for example, that traditional software architecture challenges (e.g., component coupling) also play an important role when using ML components; along with new ML specific challenges (e.g., the need for continuous retraining). Moreover, the results indicate that ML heightened decision drivers, such as privacy, play a marginal role compared to traditional decision drivers, such as scalability. Using the survey we were able to establish a link between architectural solutions and software quality attributes, which enabled us to provide twenty architectural tactics used to satisfy individual quality requirements of systems with ML components. Altogether, the results of the study can be interpreted as an empirical framework that supports the process of (re-) architecting software systems with ML components.

==> 9_articles.tex <==
\section{List of articles SLR}
\label{sec:art_list}

See Table~\ref{tbl:slr_articles}.

\onecolumn
\begin{longtable}{c|p{42em}|l}
        % \hline
        \toprule
         Source & Title & Used  \\
         \midrule
        ACM DL & A framework for managing uncertainty in software architecture & 0 \\
        ACM DL & A Report on the First Workshop on Software Engineering for Artificial Intelligence (SE4AI 2020) & 0 \\      
        ACM DL & Achieving guidance in applied machine learning through software engineering techniques & 1 \\         
        ACM DL & Deep learning UI design patterns of mobile apps & 0 \\         
        ACM DL & Designing the Software Systems of the Future & 1 \\ 
        ACM DL & Do you want to become an AI and machine learning software engineer? & 0 \\         
        ACM DL & Does fixing bug increase robustness in deep learning? & 0 \\  
        ACM DL & Emerging and Changing Tasks in the Development Process for Machine Learning Systems & 1 \\
        ACM DL & Hacking Machine Learning & 0 \\
        ACM DL & Intelligent Software Engineering: Synergy Between AI and Software Engineering &  0 \\         
        ACM DL & Keeping intelligence under control  & 0  \\         
        ACM DL & Robustness testing of autonomy software & 0 \\        
        ACM DL & Software Engineering for distributed autonomous real-time systems & 0 \\  
        ACM DL & Software Engineering for Machine Learning: A Case Study & 1 \\ 
        ACM DL & Taxonomy of real faults in deep learning systems & 0 \\         
        ACM DL & Teaching software engineering for AI-enabled systems & 0 \\         
        ACM DL & Toward a holistic software systems engineering approach for dependable autonomous systems & 1 \\        
        ACM DL &  Towards classes of architectural dependability assurance for machine-learning-based systems & 1 \\ 
        ACM DL & Tutorial on Software Testing \& Quality Assurance for Machine Learning Applications & 0 \\         
        ACM DL & Self-organizing infrastructure for machine (deep) learning at scale & 0 \\ 
        ACM DL & Sensemaking Practices in the Everyday Work of AI/ML Software Engineering & 1\\
        
        \midrule
        IEEE Xplore & A Bird's Eye View on Requirements Engineering and Machine Learning & 0 \\
        IEEE Xplore & A detailed survey of Artificial Intelligence and Software Engineering: Emergent Issues & 0 \\ 
        IEEE Xplore & A Safe, Secure, and Predictable Software Architecture for Deep Learning in Safety-Critical Systems & 0  \\ 
        IEEE Xplore & A survey of software quality for machine learning applications & 0 \\ 
        IEEE Xplore & AI Safety Landscape From short-term specific system engineering to long-term artificial general intelligence & 0 \\ 
        IEEE Xplore & Analysis of Software Engineering for Agile Machine Learning Projects  & 0 \\ 
        IEEE Xplore &  Can AI close the design-code abstraction gap? & 0 \\ 
        IEEE Xplore & Deep learning development review & 0 \\ 
        IEEE Xplore & Designing Safety Critical Software Systems to Manage Inherent Uncertainty & 1 \\ 
        IEEE Xplore & How Do Engineers Perceive Difficulties in Engineering of Machine-Learning Systems? - Questionnaire Survey & 1 \\ 
        
        IEEE Xplore & How does Machine Learning Change Software Development Practices? & 1 \\
        IEEE Xplore & Improved Self-Management Architecture in Self-Adaptive System & 0 \\ 
        IEEE Xplore & What is AI software testing? And why? & 0 \\ 
        IEEE Xplore & Requirements engineering challenges in building AI-based complex systems & 1 \\ 
        IEEE Xplore & Security engineering for machine learning & 1 \\ 
        IEEE Xplore & Software engineering challenges of deep learning & 1 \\ 
        IEEE Xplore & Software Engineering for Machine-Learning Applications: The Road Ahead & 0 \\
            IEEE Xplore & Studying Software Engineering Patterns for Designing Machine Learning Systems & 1 \\ 
        IEEE Xplore & Testing and Quality Validation for AI Software–Perspectives, Issues, and Practices & 0 \\ 
        IEEE Xplore & Towards concept based software engineering for intelligent agents & 0 \\ 
        IEEE Xplore & Uncertain requirements, assurance and machine learning & 1 \\
        IEEE Xplore & Understanding Development Process of Machine Learning Systems: Challenges and Solutions & 1 \\
        
        \midrule
        
        Science Direct & Assessing the drivers of machine learning business value & 0 \\ 
        Science Direct & AI service system development using enterprise architecture modeling & 0 \\ 
        
        \midrule
        Scopus & Big Data Analytics in Building the Competitive Intelligence of Organizations & 0 \\ 
        Scopus & Complex, Intensive Systems and Software Intelligent & 0 \\
        
        
        \midrule
        
        Google Scholar & A test architecture for machine learning product & 1 \\ 
        Google Scholar & An Analysis of ISO 26262: Using Machine Learning Safely in Automotive Software & 0 \\ 
        Google Scholar & An overview of next-generation architectures for machine learning: Roadmap, opportunities and challenges in the IoT era & 0 \\ 
        Google Scholar & SNaP ML: A hierarchical framework for machine learning & 0 \\ 
        Google Scholar & Software Architecture Design of the Real-Time Processes Monitoring Platform & 1 \\ 
        Google Scholar & Software Architecture in a Changing World & 1 \\ 
        Google Scholar & Solution Patterns for Machine Learning & 0 \\ 
        
        
        \midrule
        
        Google & A Taxonomy of Software Engineering Challenges for Machine Learning Systems: An Empirical Investigation & 1 \\ 
        Google & Continuous Delivery for Machine Learning & 1 \\
        Google & Demystifying Data Lake Architecture & 1 \\
        Google & Deploy, Connect and Execute Scientific Models & 0 \\ 
        Google & Ethics guidelines for trustworthy AI &  1 \\ 
        Google & Hidden technical debt in machine learning systems & 1\\         
        Google & The National  Artificial Intelligence Research and Development Strategic Plan: 2019 Update & 1 \\
        Google & ML Reference Architecture & 1\\ 
        Google & Machine Learning Architecture and Design Patterns & 1 \\ 
        Google & Method for Assessing the Applicability of AI Service Systems & 0 \\ 
        Google & Requirements for Trustworthy Artificial Intelligence – A Review & 1\\ 
        Google & Software Engineering Practice in the Development of Deep Learning Applications & 1 \\  
        
        
        \midrule
        Snowball & A Design Pattern for Machine Learning with Scala, Spray and Spark & 1 \\
        Snowball & AI Engineering: 11 Foundational Practices & 1\\ 
        Snowball & Adoption and Effects of Software Engineering Best Practices in Machine Learning & 1 \\
        Snowball & ClearTK 2.0: Design patterns for machine learning in UIMA & 0 \\ 
        Snowball & Continuous Training for Production ML in the TensorFlow Extended (TFX) Platform & 1 \\ 
        Snowball & Data Validation for Machine Learning & 1\\ 
        Snowball & Daisy Architecture & 1 \\
        Snowball & Expanding AI's impact with organisational learning & 0 \\ 
        Snowball & Machine learning at Facebook: Understanding inference at the edge & 1\\ 
        Snowball & Machine Learning Software Engineering in Practice: An Industrial Case Study & 1 \\
        Snowball & Machine Learning System Architectural Pattern for Improving Operational Stability & 1 \\
        Snowball & Patterns (and Anti-Patterns) for Developing Machine Learning Systems & 1 \\
        Snowball & Rules of Machine Learning & 1 \\
        Snowball & Towards using probabilistic models to design software systems with inherent uncertainty & 1 \\ 
        Snowball & Scaling distributed machine learning with the parameter server & 0 \\
        Snowball & Scaling Machine Learning as a Service & 1 \\ 
        
        \bottomrule
        \caption{Manually inspected and used articles.} 
        \label{tbl:slr_articles}                
\end{longtable}
\twocolumn

% \begin{table*}[]
%     \centering
%     \begin{tabular}{l|l|l}
%         % \hline
%         \toprule
%          Source & Title & Used  \\
%          \midrule
%         ACM DL & A framework for managing uncertainty in software architecture & 0 \\
%         ACM DL & A Report on the First Workshop on Software Engineering for Artificial Intelligence (SE4AI 2020) & 0 \\      
%         ACM DL & Achieving guidance in applied machine learning through software engineering techniques & 1 \\         
%         ACM DL & Deep learning UI design patterns of mobile apps & 0 \\         
%         ACM DL & Designing the Software Systems of the Future & 1 \\ 
%         ACM DL & Do you want to become an AI and machine learning software engineer? & 0 \\         
%         ACM DL & Does fixing bug increase robustness in deep learning? & 0 \\  
%         ACM DL & Emerging and Changing Tasks in the Development Process for Machine Learning Systems & 1 \\
%         ACM DL & Hacking Machine Learning & 0 \\
%         ACM DL & Intelligent Software Engineering: Synergy Between AI and Software Engineering &  0 \\         
%         ACM DL & Keeping intelligence under control  & 0  \\         
%         ACM DL & Robustness testing of autonomy software & 0 \\        
%         ACM DL & Software Engineering for distributed autonomous real-time systems & 0 \\  
%         ACM DL & Software Engineering for Machine Learning: A Case Study & 1 \\ 
%         ACM DL & Taxonomy of real faults in deep learning systems & 0 \\         
%         ACM DL & Teaching software engineering for AI-enabled systems & 0 \\         
%         ACM DL & Toward a holistic software systems engineering approach for dependable autonomous systems & 1 \\        
%         ACM DL &  Towards classes of architectural dependability assurance for machine-learning-based systems & 1 \\ 
%         ACM DL & Tutorial on Software Testing \& Quality Assurance for Machine Learning Applications & 0 \\         
%         ACM DL & Self-organizing infrastructure for machine (deep) learning at scale & 0 \\ 
%         ACM DL & Sensemaking Practices in the Everyday Work of AI/ML Software Engineering & 1\\
        
%         \midrule
%         IEEE Xplore & A Bird's Eye View on Requirements Engineering and Machine Learning & 0 \\
%         IEEE Xplore & A detailed survey of Artificial Intelligence and Software Engineering: Emergent Issues & 0 \\ 
%         IEEE Xplore & A Safe, Secure, and Predictable Software Architecture for Deep Learning in Safety-Critical Systems & 0  \\ 
%         IEEE Xplore & A survey of software quality for machine learning applications & 0 \\ 
%         IEEE Xplore & AI Safety Landscape From short-term specific system engineering to long-term artificial general intelligence & 0 \\ 
%         IEEE Xplore & Analysis of Software Engineering for Agile Machine Learning Projects  & 0 \\ 
%         IEEE Xplore &  Can AI close the design-code abstraction gap? & 0 \\ 
%         IEEE Xplore & Deep learning development review & 0 \\ 
%         IEEE Xplore & Designing Safety Critical Software Systems to Manage Inherent Uncertainty & 1 \\ 
%         IEEE Xplore & How Do Engineers Perceive Difficulties in Engineering of Machine-Learning Systems? - Questionnaire Survey & 1 \\ 
        
%         IEEE Xplore & How does Machine Learning Change Software Development Practices? & 1 \\
%         IEEE Xplore & Improved Self-Management Architecture in Self-Adaptive System & 0 \\ 
%         IEEE Xplore & What is AI software testing? And why? & 0 \\ 
%         IEEE Xplore & Requirements engineering challenges in building AI-based complex systems & 1 \\ 
%         IEEE Xplore & Security engineering for machine learning & 1 \\ 
%         IEEE Xplore & Software engineering challenges of deep learning & 1 \\ 
%         IEEE Xplore & Software Engineering for Machine-Learning Applications: The Road Ahead & 0 \\
%             IEEE Xplore & Studying Software Engineering Patterns for Designing Machine Learning Systems & 1 \\ 
%         IEEE Xplore & Testing and Quality Validation for AI Software–Perspectives, Issues, and Practices & 0 \\ 
%         IEEE Xplore & Towards concept based software engineering for intelligent agents & 0 \\ 
%         IEEE Xplore & Uncertain requirements, assurance and machine learning & 1 \\
%         IEEE Xplore & Understanding Development Process of Machine Learning Systems: Challenges and Solutions & 1 \\
        
%         \midrule
        
%         Science Direct & Assessing the drivers of machine learning business value & 0 \\ 
%         Science Direct & AI service system development using enterprise architecture modeling & 0 \\ 
        
%         \midrule
%         Scopus & Big Data Analytics in Building the Competitive Intelligence of Organizations & 0 \\ 
%         Scopus & Complex, Intensive Systems and Software Intelligent & 0 \\
        
        
%         \midrule
        
%         Google Scholar & A test architecture for machine learning product & 1 \\ 
%         Google Scholar & An Analysis of ISO 26262: Using Machine Learning Safely in Automotive Software & 0 \\ 
%         Google Scholar & An overview of next-generation architectures for machine learning: Roadmap, opportunities and challenges in the IoT era & 0 \\ 
%         Google Scholar & SNaP ML: A hierarchical framework for machine learning & 0 \\ 
%         Google Scholar & Software Architecture Design of the Real-Time Processes Monitoring Platform & 1 \\ 
%         Google Scholar & Software Architecture in a Changing World & 1 \\ 
%         Google Scholar & Solution Patterns for Machine Learning & 0 \\ 
        
        
%         \midrule
        
%         Google & A Taxonomy of Software Engineering Challenges for Machine Learning Systems: An Empirical Investigation & 1 \\ 
%         Google & Continuous Delivery for Machine Learning & 1 \\
%         Google & Demystifying Data Lake Architecture & 1 \\
%         Google & Deploy, Connect and Execute Scientific Models & 0 \\ 
%         Google & Ethics guidelines for trustworthy AI &  1 \\ 
%         Google & Hidden technical debt in machine learning systems & 1\\         
%         Google & The National  Artificial Intelligence Research and Development Strategic Plan: 2019 Update & 1 \\
%         Google & ML Reference Architecture & 1\\ 
%         Google & Machine Learning Architecture and Design Patterns & 1 \\ 
%         Google & Method for Assessing the Applicability of AI Service Systems & 0 \\ 
%         Google & Requirements for Trustworthy Artificial Intelligence – A Review & 1\\ 
%         Google & Software Engineering Practice in the Development of Deep Learning Applications & 1 \\  
        
        
%         \midrule
%         Snowball & A Design Pattern for Machine Learning with Scala, Spray and Spark & 1 \\
%         Snowball & AI Engineering: 11 Foundational Practices & 1\\ 
%         Snowball & Adoption and Effects of Software Engineering Best Practices in Machine Learning & 1 \\
%         Snowball & ClearTK 2.0: Design patterns for machine learning in UIMA & 0 \\ 
%         Snowball & Continuous Training for Production ML in the TensorFlow Extended (TFX) Platform & 1 \\ 
%         Snowball & Data Validation for Machine Learning & 1\\ 
%         Snowball & Daisy Architecture & 1 \\
%         Snowball & Expanding AI's impact with organisational learning & 0 \\ 
%         Snowball & Machine learning at Facebook: Understanding inference at the edge & 1\\ 
%         Snowball & Machine Learning Software Engineering in Practice: An Industrial Case Study & 1 \\
%         Snowball & Machine Learning System Architectural Pattern for Improving Operational Stability & 1 \\
%         Snowball & Patterns (and Anti-Patterns) for Developing Machine Learning Systems & 1 \\
%         Snowball & Rules of Machine Learning & 1 \\
%         Snowball & Towards using probabilistic models to design software systems with inherent uncertainty & 1 \\ 
%         Snowball & Scaling distributed machine learning with the parameter server & 0 \\
%         Snowball & Scaling Machine Learning as a Service & 1 \\ 
        
%         \bottomrule
             

%     \end{tabular}
%             \caption{Manually inspected and used articles.} 
%         \label{tbl:slr_articles}   
% \end{table*}

% \twocolumn

==> 9_data_interviews.tex <==
\section{Data Interviews}
\label{sec:data_interviewes}

See Figures~\ref{fig:data_type_int},~\ref{fig:challenges_int},~\ref{fig:challenges_dt_int}.

\begin{figure}[th]
    \centering
    \caption{Distribution of data types used by interview participants.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/data_types.pdf}
    \label{fig:data_type_int}
\end{figure}


\begin{figure}[th]
    \centering
    \caption{Distribution of architectural decision drivers from interviews.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/constraints.pdf}
    \label{fig:challenges_int}
\end{figure}


\begin{figure}[t]
    \centering
    \caption{Distribution of architectural decision drivers grouped by data type.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/constraints_datatype.pdf}
    \label{fig:challenges_dt_int}
\end{figure}




==> 9_data_slr.tex <==
\section{Data Extraction SLR}
\label{sec:slr_data}

See Table~\ref{tbl:data_items}.

\begin{table}[h]
    \centering
    \caption{Data items extracted from each article.}
    \label{tbl:data_items}
    \begin{tabular}{llp{33em}l}
    \toprule
        ID & Data Item & Description & RQ  \\
    \midrule
        1 & Title   &  The title of the article.   & Demographics \\
        
        2 & Year    &  The publication year.       & Demographics \\
        
        3 & Venue   &  The publication venue name. & Demographics \\ 
        
        4 & Context &  Academic or Industry.       & Demographics \\
        
        5 & Source  &  Retrieval source.           & Demographics \\
        
        6 & Research type & Type of research~--~\eg~validation research, evaluation research, opinion article. & Demographics. \\
        
        7 & Challenges & Documents the challenges reported in (re-) designing software with \ac{ML} components. & RQ1 \\
        
        8 & Tactics, Practices or Patterns & Documents the tactics, practices or patterns reported to meet challenges in (re-) designing software with \ac{ML} components. & RQ2 \\
        
        % 9 & Tools  & Documents the tools (if any) reported to facilitate the adoption of a tactic. & Tools \\
        
        9 & Data type & The data type used in \ac{ML}. & Data \\
        
        \bottomrule
    \end{tabular}
    
\end{table}

==> 9_demographics_slr.tex <==
\section{Demographics SLR}
\label{sec:demographics}

See Figures~\ref{fig:source_dist},~\ref{fig:year_dist},~\ref{fig:pub_dist}.

\begin{figure}[ht]
    \centering
    \caption{Distribution of manually inspected and used articles grouped by source.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/source_dist.pdf}
    \label{fig:source_dist}
\end{figure}


\begin{figure}[ht]
    \centering
    \caption{Distribution of manually inspected and used articles grouped by publication year.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/year_dist.pdf}
    \label{fig:year_dist}
\end{figure}


\begin{figure}[ht]
    \centering
    \caption{Distribution of manually inspected and used articles grouped by publication type.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/venue_dist.pdf}    
    \label{fig:pub_dist}
\end{figure}

==> 9_solutions_descriptions.tex <==
\section{Theme Description}
\label{sec:description}

\subsubsection{Run simulations to gather data.}

When designing systems with \ac{ML} components, the information regarding data, the suitable \ac{ML} techniques, or the cost of infrastructure is incomplete.
Moreover, users have unrealistic expectations regarding the quality that \ac{ML} can provide, in relation to the resources available.
To get a better understanding of the project and detect issues as early as possible, it is recommended to run simulations before defining the \ac{SA}. 
The simulations may include data flows, running \ac{ML} models on open source data that resembles the project task, deploying and scaling mock models, \etc


\subsubsection{Use past experience.}

Expert opinion and past experience can be used in designing systems with \ac{ML} components.
Nonetheless, past experience should be paired with context information, as distinct \ac{ML} techniques have different inherent requirements. 


\subsubsection{Measure and document uncertainty sources.}
To better evaluate the resources available, and create accurate expectations regarding the quality of \ac{ML} components, it is recommended to measure and document sources of uncertainty.
For example, uncertainty regarding data set size, data quality, regulatory constraints, number of users, \etc~ 
In particular, the data set size and quality may lead to bottlenecks early in the pipeline.

\subsubsection{Use metrics as functional requirements.}
Compared to traditional software, \ac{ML} components lack clear functional requirements.
To overcome this drawback, it is recommended to use concrete, measurable, metrics as functional requirements.
Examples of metrics are, accuracy, F1-score, but also metrics for trustworthy ML such as robustness, bias, \etc 


\subsubsection{Include understandability and explainability of the outputs.}

When translating requirements to measurable metrics, it is recommended to include metrics for understandability and/or explainability of the output of \ac{ML} components. 
These metrics help to analyse and understand the data and the \ac{ML} components.
Moreover, they help shape future decisions such as choosing \ac{ML} techniques suitable for the task, fall-back mechanisms, n-versioning, \etc


\subsubsection{Analyse regulatory constraints up-front.}

Although \ac{ML}/AI specific regulatory constraints are, at the moment, in draft phase, their impact on systems with \ac{ML} component is expected to grow in the near future.
By analysing the regulatory constraints upfront, architects can prepare the system for compliance and audits.
For example, regulatory constraints may enforce privacy requirements, which will translate to \ac{SA} decisions for using privacy preserving \ac{ML} techniques, privacy data management methods, \etc 


\subsubsection{Adopt an AI code of conduct.}
AI code of conducts help shape both a system and the organisation.
For example, a code of conduct can stipulate the responsible use of ML/AI, which will translate to \ac{SA} decisions for using interpretable models.
Organisation wise, AI code of conducts will guide the decision processes.


\subsubsection{Design audit trails.}
Audit trails help to analyse and understand a system, even without context knowledge.
Since \ac{ML} components are intrinsically opaque, it is recommended to think of audit traces when defining the \ac{SA}. 
This process will help to define separate models to aggregate logs, provide visualisations, or automate reports and audit traces.
Moreover, it helps third parties to assess compliance to regulatory constraints.



\subsubsection{Design separate modules/services for data collection and data preparation.}

Data collection and preparation are experimental processes, which may result in a jungle of scrapes, joins and sampling steps.
Therefore, the modularity and reuse of data modules is diminished.
In order to avoid high coupling and facilitate code reuse, it is recommended to separate data collection and preparation into separate modules, which can be imported/deployed and orchestrated independently.


\subsubsection{Integrate external tools for data collection and preparation.}

Multiple tools already provide data collection and preparation capabilities (\eg~Snorkel\footnote{https://www.snorkel.org/}). 
In case the project does not have tight data management constraints (\eg~privacy), architects can choose to integrate external tools.
When choosing the tools for these task, architects must ensure they can be integrated with the system, and orchestrated in different services.

\subsubsection{Design separate modules/services for data quality assessment.}

Data quality assessment consists of testing the data for missing data values, distribution skews, drifts, \etc~In order to avoid coupling between data components, it is recommended to separate data quality assessment in individual modules/services. 
The modules should be independently imported/deployed and integrated in multiple pipelines, ensuring modularity and reusability.


\subsubsection{Standardise model interfaces.}

To facilitate interoperability and reusability between training and serving, it is recommended to package \ac{ML} models in standard interfaces.
Choosing an interface type is project specific, and can include REST APIs, gRPCs, etc.
Nonetheless, the models' interfaces should be the same as the interfaces for other components in the system.


\subsubsection{Use one middleware.}
To enhance interoperability between \ac{ML} and other components, and better integrate the \ac{ML} experimental work-flow with traditional software, it is recommended to use a communication middleware between components.
Even more, the middleware can be reused between training and serving, because the impact from training on infrastructure should not be high.
For example, if the system uses a message queue in production, thee number of messages exchanged for training will be small.

\subsubsection{Reuse virtualisation and infrastructure scripts.}

Infrastructure-as-code and virtualisation (\eg~Docker) should be adopted in all systems with \ac{ML} components.
Moreover, this code for infrastructure and virtualisation can be reused between training and serving, \eg~by holding states in configuration files.



\subsubsection{Separate business logic from \ac{ML} components.}

To distinguish errors between \ac{ML} components and business logic, it is recommended to separate their concerns and development.
The separation can be done by using independent modules/services for each concern.
Moreover, standardisation of interfaces and the use of one middleware facilitate interoperation between business logic and \ac{ML} components.


\subsubsection{Standardise interfaces.}

As mentioned in \emph{standardise model interfaces}, standardisation of interfaces should be adopted between all components in a system.


\subsubsection{Design independent modules/services for ML and data.}

\ac{ML} components are coupled (and dependent) to data components.
To minimise the coupling between the two, it is recommended to design independent modules or services for \ac{ML} models and data (as also recommended in the data category).


\subsubsection{Relax coupling heuristics between ML and data.}

Since \ac{ML} and data components are highly coupled, there are use cases when the coupling can not be reduced.
Therefore, for \ac{ML} components it is recommended to relax coupling heuristics.
Nonetheless, the heuristics should not be relaxed for other (business) logic.


\subsubsection{Use n-versioning.}
Ensembles of \ac{ML} models are used to decrease the risk of over-fitting, better approximate prediction uncertainty or facilitate interpretability. 
Thinking of ensembles as n-versioning helps to understand the role of each model, and its integration in the system.
Moreover, it helps to separate the voting logic from the \ac{ML} logic. 
An example is using an interpretable or rule based model as back-up for a black-box model. 

\subsubsection{Design and monitor uncertainty measures.}

Besides the metrics used as functional requirements (\eg~accuracy), it is recommended to monitor the uncertainty of \ac{ML} components because it can signal degradation of models and silent failures.

\subsubsection{Employ interpretable models.}
Interpretable models help to understand the decisions of \ac{ML} components both by developers and users.
Therefore, they should be the first choice for all systems with \ac{ML} components.
In case interpretable models can not satisfy functional requirements, they should be developed as secondary models in n-versioning.


\subsubsection{Use human intervention.}

If possible, \ac{ML} models should be assessed by team members (\eg~developers, data scientists, \etc).



\subsubsection{Use metric monitoring and alerts to detect failures.}
\ac{ML} components can fail silently, \ie~their predictions can be erroneous, in spite of the fact that they are running.
To detect silent failures, it is recommended to use continuous monitoring of metrics, and implement alert systems which can notify incidents (\eg~decrease in accuracy, increase in uncertainty).
When designing the alert modules, it is important to consider that alerts may be interpreted by team members that did not assisted the development.
Therefore, alerts should be comprehensive enough to be interpreted by external actors.


\subsubsection{Instrument the system to the fullest extent.}

Instrumentation is key to detection of failures, distribution shifts, or, more generally, malfunctions of \ac{ML} components.
Therefore, it is recommended to dedicate attention to define as many metric as possible, in order to analyse \ac{ML} components.
Instrumentation also facilitates incident management in production.


\subsubsection{Design log modules to aggregate metrics.}

Log modules should be designed to allow fast mining of data.
Nonetheless, in preparation for time constrained situations, such as incident management, log modules should be designed to already aggregate metrics and save high level conclusions.
Aggregates are also helpful for audit reports.


\subsubsection{Design log modules to visualise metrics.}

Besides metric aggregation, the design of visualisations modules to monitor \ac{ML} components is recommended.



\subsubsection{Wrap components in APIs/modules/services.}

Using generic packages for \ac{ML}  can result in large amounts of support code that connects  \ac{ML} components to other parts of the system.
This glue code is costly, because it makes systems dependent on packages versions.
To combat glue code, black-box packages can be wrapped in common APIs or independent modules/services.


\subsubsection{Version configuration files.}

To reproduce previous \ac{ML} experiments, and collect historical data about successful experiments, it is recommended to version configuration files among other artefacts, such as training and testing data, or models.


\subsubsection{Design the log system to support AutoML}

Data supporting the automation of \ac{ML} development can be collected from logging or versioning. 
Designing the log system to support AutoML consists of designing modules for data storage and retrieval. 
An example is the creation of data sinks to support AutoML.

\subsubsection{Design the version system to support AutoML}

Similar to designing the logging system to support AutoML, the versioning system can support data collection and retrieval for AutoML. 
For example, by creating repositories dedicated to AutoML data.

\subsubsection{Design model tests.}

Model testing are similar to unit tests, but for \ac{ML} models.
Model tests verify if models work with the data used in serving, and if their output satisfy predefined conditions.
Besides implementing the tests, it is recommended to encapsulate them in independent modules, which can be orchestrated in different processes, if needed. 

\subsubsection{Design data tests.}
Data tests check the data satisfies predefined conditions; such as format, missing fields, distributions, \etc~
Similar to model tests, data tests should be encapsulated in independent modules, which can be reused in multiple pipelines.
Moreover, it is desired to reuse data tests between training and pipelines.


\subsubsection{Use integration tests.}

Integration tests verify the integration of \ac{ML} components with other components in the system, and prevent cascading errors.
Therefore, they are recommended for all systems with \ac{ML} components.


\subsubsection{Use CI/CD.}

Automation in building, testing and deployment of systems with \ac{ML} components facilitates fault isolation, increases reliability and team agility.
Therefore, CI/CD is recommended for all projects with \ac{ML} components.

\subsubsection{Use unit tests.}

Besides model and data tests, it is recommended to write unit tests for all code; as in traditional software development.


\subsubsection{Use data ownership for test modules.}

Consider individual data splits owned by test modules. 
In this way, one can ensure that test data is not mistakenly used for training.
Moreover, test modules orchestrated in different pipelines will rely on independent data samples.
However, it is recommended to ensure the data is continuously refreshed.

\subsubsection{Use metrics and CI/CD for validation.}

In order to validate models for production, it is recommended to design a metric suite, and automate its verification through CI/CD.


\subsubsection{Use alerts for validation.}

In case a model is promoted/discarded for production, it is recommended to announce it to the team through an alert module.


\subsubsection{Use human intervention for validation.}

In order to maintain human oversight, it is recommended that team members analyse models promoted to production.


\subsubsection{Design for automatic continuous retraining.}

Maintenance an evolution of \ac{ML} components requires continuous retraining.
In is recommended to design the system s.t. this process can be  automated.
For example, by developing modules that can deploy infrastructure and orchestrate data and training modules.


% \subsubsection{Use CI/CD for maintenance.}

% To promote newly trained models to production, it is recommended to use CI/CD.

\subsubsection{Use automatic rollback.}

If, due to changes in the input data or undetected skew, a deployed model performs sub-optimal, it should be rolled back to an earlier, better performing version.
Designing a process for automatic roll-back minimizes the time a deployed model with sub-optimal performance is kept in production.


\subsubsection{Use infrastructure-as-code.}

Setting up the infrastructure for \ac{ML} components (\eg~starting new machines, transferring the data) is a tedious process.
In order to increase the agility, it is recommended to automate this task.

\subsubsection{Adopt standard release processes.}

To avoid human errors and sub-optimal models from being deployed, it is recommended to design and adopt standard releases processes.
Since \ac{ML} teams are heterogeneous, some team members may be unaware of the processes for model release or roll-back. 
Shared within the team, standard processes empower members to act when faced with incidents.


\subsubsection{Encapsulate ML components in identifiable modules/services.}

To manage the dependencies and consumers of \ac{ML} components, it is recommended to encapsulate them in identifiable modules/services.
The unique identifiers can be used to trace back consumers, and should be used to log all interactions with \ac{ML} components. 

\subsubsection{Use authentication and access control.}

In order to forbid access to \ac{ML} consumers, it is recommended to implement authentication and access control policies.
Similar policies should be implement for the data used by \ac{ML} components.


\subsubsection{Log consumers of ML consumers.}

Unique identifiers of \ac{ML} components can be used to trace back consumers, and should be used to log for all interactions with \ac{ML} components. 


\subsubsection{Design for batch processing for training and stream processing for serving.}

To balance latency, throughput, and fault-tolerance, needed for training and serving it is recommended to adopt a lambda architecture, \ie~use batch processing for training and stream processing for serving.

\subsubsection{Physically isolate the workloads.}

To scale training and serving workloads, it is recommended to physically isolate them, \ie~deploy on distinct physical hardware.
This is automatically done when using cloud services.


\subsubsection{Use virtualisation.}

To abstract from the software suite needed for \ac{ML}, and increase reproducibility and agility, it is recommended to use virtualisation (\eg~Docker).


\subsubsection{Design for traceability and reproducibility.}

In a system with \ac{ML} components, traceability and reproducibility are inherent requirements which need to be satisfied.
Different strategies can be applied, within which two methods are common: logging pointers to versioned artefacts, and versioning of data and model related artefacts.



\subsubsection{Log pointers to versioned artefacts.}

Tracing decisions back to the input data and the model's version can be difficult. 
It is therefore recommended to log production predictions together with the model's version and input data.


\subsubsection{Version configurations, models and data}

To reproduce previous \ac{ML} experiments, one needs more than just the executable code. Versioning the training and testing data, the final model, and all configuration files is complementary to versioning the code.


\subsubsection{Form multi-disciplinary teams.}

\ac{ML} components require the integration of different technology stacks responsible for infrastructure, data management, model training and serving.
To tackle the challenges at different levels, it is recommended to form multi-disciplinary teams consisting of members responsible for different levels of the stack.


\subsubsection{Define processes for decision making.}

In many cases, decisions have to be made under uncertainty and incomplete information. 
To enhance the ability of a team to make the right decisions at the right time, it is recommended to define and enforce a standard process across team members.
\ac{ML} adds more uncertainty to a system, and increases the importance of standard processes for decision making. 

\subsubsection{Raise awareness of \ac{ML} risks within the team.}

Even when used with good intentions, \ac{ML} can negatively impact on the society. 
Therefore, it is recommended to inform team members working at different levels of the stack about \ac{ML} risks.



==> 9_solutions_interviews.tex <==
\section{Solutions after the interviews}
\label{sec:solutions_interviews}
See Table~\ref{tbl:practices_interviews}.

% 61
\begin{table*}[ht]
	\caption{List of \ac{SA} challenges and solutions after the interviews.}
	
	\label{tbl:practices_interviews}
	\begin{tabular}{p{1em}p{3em}p{22em}p{22em}p{4em}}
    \toprule
		Nr. & Category & Challenges & Solutions  & References  \\
    \midrule
        1 & Reqs. & At design time the information available is insufficient to understand the customers or the projects. &
        Run simulations to gather data. Use past experience. Measure and document  uncertainty sources.
        % Identify sources of uncertainty, measure and document them. Run experiments and use past experience.  
        & \cite{ishikawa2019engineers,belani2019requirements,chechik2019uncertain, lwakatare2019taxonomy,wan2019does,liu2020emerging} \\ 

        2 & Reqs. & \ac{ML} components lack functional requirements. & 
        Use metrics as functional requirements. Include understandability and explainability of the outputs.
        % Choose concrete, measurable, metrics. Include understandability and explainability of the outputs.
        & \cite{ishikawa2019engineers,belani2019requirements,lwakatare2019taxonomy,de2019understanding,wan2019does,chechik2019uncertain} \\ 
        
        
        3 & Reqs. & \ac{ML} projects have regulatory restrictions and may be subject to audits. & 
        % Analyse regulatory constraints up-front. Design audit trails.
        Analyse regulatory constraints up-front. Adopt an AI code of conduct. Design audit trails.
        & \cite{kaur2020requirements,national2019national,MLRARCH,serban2020adoption} \\
        
        \midrule
        
        4 & Data & Data preparation may result in a jungle of scrapes, joins, and sampling steps, often with intermediate outputs. & 
        % Design separate modules/services for data collection and data preparation. Encapsulate for reuse. 
        Design separate modules/services for data collection and data preparation. Integrate external tools. 
        & \cite{sculley2015hidden,li2017scaling,de2019understanding} \\ 
        
        
        5 & Data & Data quality is hard to test, and may have unexpected consequences. & 
        % Design separate modules/services for data testing. Encapsulate for reuse.
        Design separate modules/services for data quality assessment. Integrate external tools.
        & \cite{zhang2019software, polyzotis2019data,li2017scaling,mcgraw2019security,de2019understanding} \\
        
        \midrule
        
        6 & Design & Separate concerns between training, testing, and serving, but reuse code between them. & 
        Standardise model interfaces. Use one middleware. Reuse virtualisation, infrastructure and test scripts.
        % Use one  middleware and standardised interfaces.% for both pipelines. 
        % Design separate modules/services. Encapsulate for reuse. 
        & \cite{amershi2019software,RLML,wu2019machine} \\ 
        
        7 & Design & Distinguish failures between \ac{ML} components and other business logic. &
        Separate business logic from ML components. Standardise interfaces and use one middleware between them.
        % Separate business logic from ML development. Use standardised interfaces and middleware between the two.
        & \cite{yokoyama2019machine,rahman2019machine} \\           
        
        8 & Design & ML components are highly coupled, and errors can have cascading effects. 
        % For instance, the performance of data modeling is dependent on data collection.  
        & 
        Design independent modules/services for \ac{ML} and data. Standardise interfaces and use one middleware. Relax coupling heuristics between \ac{ML}  and data. 
        % Decouple components using independent modules/services. Encapsulate for reuse. Relax design heuristics between \ac{ML} and data.
        & \cite{wan2019does,northrop2019designing,horneman2020ai} \\ 
        
        
        9 & Design &  \ac{ML} components bring inherent uncertainty to a system. & 
        Use n-versioning. Design and monitor uncertainty metrics. Employ interpretable models/human intervention. Use self adaptation.
        & \cite{aniculaesei2018toward,northrop2019designing,serban2019designing,serban2020towards,horneman2020ai} \\
        
        10 & Design & ML components can fail silently. 
        % (i.e. have high uncertainty or under-perform). 
        These failures can be hard to detect, isolate and solve. 
        % because they are different from bugs that crash the software. 
        & 
        Use metric monitoring and alerts to detect failures. Use n-versioning. Employ interpretable models. Detect out of distrribution data.
        % Design metrics to detect failures. Use interpretable models. Use n-versioning. 
        & \cite{biondi2019safe, serban2019designing, woods2016software} \\
        
        11 & Design & \ac{ML} components are intrinsically opaque, and deductive reasoning from the architecture artefacts, code or metadata is not effective. 
        % in reasoning about the system / components. 
        & Instrument the system to the fullest extent. Use n-versioning. Employ interpretable models. Design log modules to aggregate/visualise metrics.
        % Instrument the system to the fullest extent. Design log modules to aggregate metrics, enable visualisations and alerts. Use interpretable models and n-versioning.
        & \cite{scheerer2020towards,northrop2019designing,horneman2020ai,RLML} \\
        
        
        12 & Design & Avoid unstructured components which link frameworks or APIs (\eg~glue code). & Wrap components in APIs/modules/services. Use standard interfaces and one middleware. Use virtualisation. & 
        \cite{sculley2015hidden} \\      
        
        
        13 & Design & Automation and understanding of \ac{ML} tasks is difficult (AutoML).
         & Version configuration files. Design the log and versioning systems to support AutoML data retrieval.
        %  Design versioning and logging modules for experiment data (configurations, models, data). Create automated checkpoints, documentation and reports for audits.
         & \cite{wan2019does,li2017scaling,wu2019machine,serban2020adoption,PAPML} \\        
        
        \midrule
    
        
        14 & Testing & \ac{ML} testing goes beyond programming bugs to issues that arise from model, data errors, or uncertainty. &  
        Design model and data tests. Use CI/CD. Use integration and unit tests. Use data ownership for test modules. Use manual inspection.
        % Design separate test modules (for model, data, unit and integration tests). Encapsulate for reuse and automation (CI). Consider data splits ownership for each module. 
        & 
        \cite{arpteg2018software,amershi2019software,nishi2018test,zhang2019software,reimann2020achieving}  \\
        % Ideally the testing and validation components are independent from training, and own the test/validation data set (i.e., this daa split is not available to any other component). Ideally this component can be deployed independently and reused / integrated / orchestrated.
        
        15 & Testing & Validation of \ac{ML} components for production is difficult. & 
        Use metrics and CI/CD for validation.  Use alerts, visualisations, human intervention. Design release processes. 
        % Use automatic validation (CD). Design visualisation and alert modules. Standardise release processes. 
        &  \cite{CD4ML}  \\ 
        
        
        \midrule
        
        16 & Ops. & ML components require continuous maintenance, retraining and evolution. & 
        Design for automatic continuous retraining. Use CI/CD. Use automatic rollback. Use infrastructure-as-code. Adopt standard release processes.
        % Design for evolution with continuous (re-) training and deployment, automatic documentation, deployment and rollback, CI/CD, infrastructure-as-code.
        % E.g. having a central repository with model cards, and decision records (similar to architecture decision records).
        & \cite{CD4ML,CTPML,northrop2019designing,washizaki2019studying,wan2019does,zhang2019software,liu2020emerging} \\ 
        
        
        17 & Ops. & Manage the dependencies and consumers of ML applications. & 
         Encapsulate \ac{ML} components in identifiable modules/services. Use authentication and access control. Log consumers of \ac{ML} components.
        %  Encapsulate \ac{ML} components for reuse in modules/services. Use virtualisation. Implement authentication and access restrictions. Log \ac{ML} consumers.
        %  For example, use architectural styles such as event driven or microservices. Access restrictions and logging the access to models helps to avoid undeclared consumers.
         & \cite{sculley2015hidden,DACH,yokoyama2019machine,batyuk2018software,horneman2020ai} \\         
        
        18 & Ops. & Balance latency, throughput, and fault-tolerance, needed for training and serving. & 
        Design for batch processing (training) and stream processing (serving), \ie~lambda architecture. Physically isolate the workloads. Use virtualisation.
        % Design for batch processing (training) and stream processing (serving), \ie~lambda architecture. Use virtualisation and physically isolate the workloads. 
        & \cite{li2017scaling,DMLA,washizakimachine, wu2019machine,ADPML} \\
        
        
         
        19 & Ops. & Trace back decisions to models, data and reproduce past results. & 
        Design for traceability and reproducibility; log pointers to versioned artefacts, version configurations, models and data.
        % Design for traceability and reproducibility; version configuration files and pointers to models and data. Log the pointers with production predictions. 
        & P10   \\          
         
        
        \midrule
        
        20 & Org. & \ac{ML} applications use heterogeneous technology stacks which require diverse backgrounds and skills.  & 
        Form multi-disciplinary teams. Adopt an AI code of conduct. Define processes for decision-making. Raise awareness about \ac{ML} risks within the team.
        % Form multi-disciplinary teams for \ac{ML}. Define processes for decision-making. Adopt a code of conduct and raise awareness about risks of using \ac{ML} within the team.  
        & P1 \\

    \bottomrule 
    \end{tabular}
\end{table*}


==> 9_solutions_slr.tex <==
\section{Solutions extracted from the SLR}
\label{sec:solutions_slr}
See Table~\ref{tbl:practices_slr}.
% 61
% 29 solutions
\begin{table*}[ht]
	\caption{List of \ac{SA} challenges for \ac{ML} and related solutions as extracted from the SLR.}
	
	\label{tbl:practices_slr}
	\begin{tabular}{p{1em}p{3em}p{22em}p{22em}p{4em}}
    \toprule
		Nr. & Category & Challenges & Solutions  & References  \\
    \midrule
        1 & Reqs. & At design time the information available is insufficient to understand the customers or the projects. & Measure and document uncertainty sources.
        % Identify sources of uncertainty, measure and document them. Run experiments and use past experience.  
        & \cite{ishikawa2019engineers,belani2019requirements,chechik2019uncertain, lwakatare2019taxonomy,wan2019does,liu2020emerging} \\ 

        2 & Reqs. & \ac{ML} components lack functional requirements. & 
        Use metrics as functional requirements. Include understandability and explainability of the outputs.
        % Choose concrete, measurable, metrics. Include understandability and explainability of the outputs.
        & \cite{ishikawa2019engineers,belani2019requirements,lwakatare2019taxonomy,de2019understanding,wan2019does,chechik2019uncertain} \\ 
        
        
        3 & Reqs. & \ac{ML} projects have regulatory restrictions and may be subject to audits. & 
        % Analyse regulatory constraints up-front. Design audit trails.
        Analyse regulatory constraints up-front. Adopt an AI code of conduct. Design audit trails.
        & \cite{kaur2020requirements,national2019national,MLRARCH,serban2020adoption} \\
        
        \midrule
        
        4 & Data & Data preparation may result in a jungle of scrapes, joins, and sampling steps, often with intermediate outputs. & 
        % Design separate modules/services for data collection and data preparation. Encapsulate for reuse. 
        Design separate modules/services for data collection and data preparation. 
        & \cite{sculley2015hidden,li2017scaling,de2019understanding} \\ 
        
        
        5 & Data & Data quality is hard to test, and may have unexpected consequences. & 
        % Design separate modules/services for data testing. Encapsulate for reuse.
        Design separate modules/services for data quality assessment.
        & \cite{zhang2019software, polyzotis2019data,li2017scaling,mcgraw2019security,de2019understanding} \\
        
        \midrule
        
        6 & Design & Separate concerns between training, testing, and serving, but reuse code between them. & 
        Standardise model interfaces. 
        % Use one  middleware and standardised interfaces.% for both pipelines. 
        % Design separate modules/services. Encapsulate for reuse. 
        & \cite{amershi2019software,RLML,wu2019machine} \\ 
        
        7 & Design & Distinguish failures between \ac{ML} components and other business logic. &
        Separate business logic from ML components. 
        % Separate business logic from ML development. Use standardised interfaces and middleware between the two.
        & \cite{yokoyama2019machine,rahman2019machine} \\           
        
        8 & Design & ML components are highly coupled, and errors can have cascading effects. 
        % For instance, the performance of data modeling is dependent on data collection.  
        & 
        Design independent modules/services for \ac{ML} and data. Relax coupling heuristics between \ac{ML}  and data. 
        % Decouple components using independent modules/services. Encapsulate for reuse. Relax design heuristics between \ac{ML} and data.
        & \cite{wan2019does,northrop2019designing,horneman2020ai} \\ 
        
        
        9 & Design &  \ac{ML} components bring inherent uncertainty to a system. & 
        Design and monitor uncertainty metrics. 
        %  Separate \ac{ML} components based on expected uncertainty. Use n-versioning. Monitor uncertainty.
        & \cite{aniculaesei2018toward,northrop2019designing,serban2019designing,serban2020towards,horneman2020ai} \\
        
        10 & Design & ML components can fail silently. 
        % (i.e. have high uncertainty or under-perform). 
        These failures can be hard to detect, isolate and solve. 
        % because they are different from bugs that crash the software. 
        & 
        Use metric monitoring and alerts to detect failures. 
        % Design metrics to detect failures. Use interpretable models. Use n-versioning. 
        & \cite{biondi2019safe, serban2019designing, woods2016software} \\
        
        11 & Design & \ac{ML} components are intrinsically opaque, and deductive reasoning from the architecture artefacts, code or metadata is not effective. 
        % in reasoning about the system / components. 
        & Instrument the system to the fullest extent. Design log modules to aggregate/visualise metrics.
        % Instrument the system to the fullest extent. Design log modules to aggregate metrics, enable visualisations and alerts. Use interpretable models and n-versioning.
        & \cite{scheerer2020towards,northrop2019designing,horneman2020ai,RLML} \\
        
        
        12 & Design & Avoid unstructured components which link frameworks or APIs (\eg~glue code). & Wrap components in APIs/modules/services.  & 
        \cite{sculley2015hidden} \\      
        
        
        13 & Design & Automation and understanding of \ac{ML} tasks is difficult (AutoML).
         & Version configuration files. Design the log and versioning systems to support AutoML data retrieval.
        %  Design versioning and logging modules for experiment data (configurations, models, data). Create automated checkpoints, documentation and reports for audits.
         & \cite{wan2019does,li2017scaling,wu2019machine,serban2020adoption,PAPML} \\        
        
        \midrule
    
        
        14 & Testing & \ac{ML} testing goes beyond programming bugs to issues that arise from model, data errors, or uncertainty. &  
        Design model and data tests. Use CI/CD. 
        % Design separate test modules (for model, data, unit and integration tests). Encapsulate for reuse and automation (CI). Consider data splits ownership for each module. 
        & 
        \cite{arpteg2018software,amershi2019software,nishi2018test,zhang2019software,reimann2020achieving}  \\
        % Ideally the testing and validation components are independent from training, and own the test/validation data set (i.e., this daa split is not available to any other component). Ideally this component can be deployed independently and reused / integrated / orchestrated.
        
        15 & Testing & Validation of \ac{ML} components for production is difficult. & 
        Use metrics and CI/CD for validation.  Use alerts, visualisations.
        % Use automatic validation (CD). Design visualisation and alert modules. Standardise release processes. 
        &  \cite{CD4ML}  \\ 
        
        
        \midrule
        
        16 & Ops. & ML components require continuous maintenance, retraining and evolution. & 
        Design for automatic continuous retraining. Use CI/CD. Use automatic rollback.
        % Design for evolution with continuous (re-) training and deployment, automatic documentation, deployment and rollback, CI/CD, infrastructure-as-code.
        % E.g. having a central repository with model cards, and decision records (similar to architecture decision records).
        & \cite{CD4ML,CTPML,northrop2019designing,washizaki2019studying,wan2019does,zhang2019software,liu2020emerging} \\ 
        
        
        17 & Ops. & Manage the dependencies and consumers of ML applications. & 
         Use authentication and access control. Log consumers of \ac{ML} components.
        %  Encapsulate \ac{ML} components for reuse in modules/services. Use virtualisation. Implement authentication and access restrictions. Log \ac{ML} consumers.
        %  For example, use architectural styles such as event driven or microservices. Access restrictions and logging the access to models helps to avoid undeclared consumers.
         & \cite{sculley2015hidden,DACH,yokoyama2019machine,batyuk2018software,horneman2020ai} \\         
        
        18 & Ops. & Balance latency, throughput, and fault-tolerance, needed for training and serving. & 
        Design for batch processing (training) and stream processing (serving), \ie~lambda architecture. Physically isolate the workloads. 
        % Design for batch processing (training) and stream processing (serving), \ie~lambda architecture. Use virtualisation and physically isolate the workloads. 
        & \cite{li2017scaling,DMLA,washizakimachine, wu2019machine,ADPML} \\

    \bottomrule 
    \end{tabular}
\end{table*}


==> 9_survey.tex <==
\section{Solutions from survey}
\label{sec:survey_solutions}

See Figure~\ref{fig:ss1}~-~\ref{fig:ss20}.

%%% 1.
\begin{figure}[th]
    \centering
    \caption{Survey solutions to practice 1.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/req_lack_info.pdf}
    \label{fig:ss1}
\end{figure}


%%% 2.
\begin{figure}[th]
    \centering
    \caption{Survey solutions to practice 2.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/req_lack_reqs.pdf}
    \label{fig:ss2}
\end{figure}


%%% 3.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 3.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/req_regulatory.pdf}
    \label{fig:ss3}
\end{figure}


%%% 4.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 4.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/data_collection.pdf}
    \label{fig:ss4}
\end{figure}


%%% 5.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 5.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/data_quality.pdf}
    \label{fig:ss5}
\end{figure}


%%% 6.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 6.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_code_reuse.pdf}
    \label{fig:ss6}
\end{figure}


%%% 7.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 7.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_business_logic.pdf}
    \label{fig:ss7}
\end{figure}


%%% 8.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 8.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_component_coupling.pdf}
    \label{fig:ss8}
\end{figure}


%%% 9.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 9.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_uncertainty.pdf}
    \label{fig:ss9}
\end{figure}


%%% 10.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 10.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_ml_failures.pdf}
    \label{fig:ss10}
\end{figure}


%%% 11.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 11.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_opaqueness.pdf}
    \label{fig:ss11}
\end{figure}



%%% 12.

\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 12.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_unstructured.pdf}
    \label{fig:ss12}
\end{figure}


%%% 13.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 13.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_automl.pdf}
    \label{fig:ss13}
\end{figure}



%%% 14.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 14.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/test_test.pdf}
    \label{fig:ss14}
\end{figure}



%%% 15.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 15.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/test_validation.pdf}
    \label{fig:ss15}
\end{figure}



%%% 16.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 16.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/ops_maintenance.pdf}
    \label{fig:ss16}
\end{figure}


%%% 17.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 17.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/ops_consumers.pdf}
    \label{fig:ss18}
\end{figure}


%%% 18.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 18.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/ops_latency.pdf}
    \label{fig:ss18}
\end{figure}


%%% 19.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 19.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/ops_traceability.pdf}
    \label{fig:ss19}
\end{figure}



%%% 20.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to practice 20.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/org.pdf}
    \label{fig:ss20}
\end{figure}


%%% 20.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to instrumentation.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/design_instrumentation.pdf}
    \label{fig:ssinstrument}
\end{figure}


%%% 20.
\begin{figure}[H]
    \centering
    \caption{Survey solutions to interview challenges, grouped by team size.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/interview_challenge.pdf}
    \label{fig:interview_challenge}
\end{figure}



==> 9_survey_demographics.tex <==
\section{Survey demographics}
\label{sec:survey_demographics}

%%% 1.
\begin{figure}[h]
    \centering
    \caption{Organisation type for survey participants.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/org_type.pdf}
    \label{fig:survey_org_type}
\end{figure}


%%% 2.
\begin{figure}[th]
    \centering
    \caption{Experience of survey participants.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/experience.pdf}
    \label{fig:survey_exp}
\end{figure}



%%% 3.
\begin{figure}[t]
    \centering
    \caption{Team size for survey participants.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/team_size.pdf}
    \label{fig:survey_org_type}
\end{figure}


%%% 4.
% \begin{figure}[t]
%     \centering
%     \caption{Decision drivers for survey participants.}
%     \includegraphics[width=7cm, keepaspectratio]{figures/survey/decision_drivers.pdf}
%     \label{fig:survey_decision_drivers}
% \end{figure}


%%% 5.
\begin{figure}[t]
    \centering
    \caption{Data types used by survey participants.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/data_types.pdf}
    \label{fig:survey_data_types}
\end{figure}



%%% 6.
\begin{figure}[t]
    \centering
    \caption{Deployment interval for survey participants.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/deployment_interval.pdf}
    \label{fig:survey_deployment}
\end{figure}


%%% 7.
\begin{figure}[t]
    \centering
    \caption{Regions for survey participants.}
    \includegraphics[width=7cm, keepaspectratio]{figures/survey/region.pdf}
    \label{fig:survey_regions}
\end{figure}

==> 9_themes_interviews.tex <==
\section{Themes extracted from interviews}
\label{sec:themes_interviews}

%%% 1.
\begin{figure}[th]
    \centering
    \caption{Themes extracted for challenge 1.}    
    \includegraphics[width=8cm, keepaspectratio]{figures/interviews/themes/data_design.pdf}
    \label{fig:ch_1}
\end{figure}

%%% 2.
\begin{figure}[th]
    \centering
    \caption{Themes extracted for challenge 2.}    
    \includegraphics[width=8cm, keepaspectratio]{figures/interviews/themes/func_reqs.pdf}
    \label{fig:ch_1}
\end{figure}


%%% 4.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 4.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/data_prep.pdf}
    \label{fig:ch_4}
\end{figure}


%%% 5.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 5.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/data_valid.pdf}
    \label{fig:ch_5}
\end{figure}


%%% 6.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 6.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/code_reuse.pdf}
    \label{fig:6}
\end{figure}



%%% 7.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 7.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/business_logic.pdf}
    \label{fig:ch_7}
\end{figure}


%%% 8.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 8.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/coupling.pdf}
    \label{fig:ch_8}
\end{figure}


%%% 9.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 9.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/inh_uncertainty.pdf}
    \label{fig:ch_9}
\end{figure}


%%% 10.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 10.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/ml_failures.pdf}
    \label{fig:ch_9}
\end{figure}



%%% 11.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 11.}       \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/monitoring.pdf}
    \label{fig:ch_9}
\end{figure}



%%% 12.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 12.}   
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/differences_tr_test.pdf}
    \label{fig:ch_9}
\end{figure}


%%% 13.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 13.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/automl.pdf}
    \label{fig:ch_9}
\end{figure}


%%% 14.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 14.}
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/testing.pdf}
    
    \label{fig:ch_9}
\end{figure}



%%% 15.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 15.}    
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/human_intervention.pdf}
    \label{fig:ch_9}
\end{figure}


%%% 16.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 16.}
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/maintenance.pdf}
    \label{fig:ch_9}
\end{figure}


%%% 17.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 17.}
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/consumers.pdf}
    \label{fig:ch_9}
\end{figure}


%%% 18.
\begin{figure}[t]
    \centering
    \caption{Themes extracted for challenge 18.}
    \includegraphics[width=9cm, keepaspectratio]{figures/interviews/themes/glue_code.pdf}
    \label{fig:ch_9}
\end{figure}


==> questions.tex <==
% .” Architecture is about the important stuff. Whatever that is. - who needs an architect
% What is the most important element of architecting with ML?






